Dead or Murdered? Predicting Responsibility Perception in Femicide News Reports

Different linguistic expressions can conceptualize the same event from different viewpoints by emphasizing certain participants over others. Here, we investigate a case where this has social consequences: how do linguistic expressions of gender-based violence (GBV) influence who we perceive as responsible? We build on previous psycholinguistic research in this area and conduct a large-scale perception survey of GBV descriptions automatically extracted from a corpus of Italian newspapers. We then train regression models that predict the salience of GBV participants with respect to different dimensions of perceived responsibility. Our best model (fine-tuned BERT) shows solid overall performance, with large differences between dimensions and participants: salient _focus_ is more predictable than salient _blame_, and perpetrators' salience is more predictable than victims' salience. Experiments with ridge regression models using different representations show that features based on linguistic theory similarly to word-based features. Overall, we show that different linguistic choices do trigger different perceptions of responsibility, and that such perceptions can be modelled automatically. This work can be a core instrument to raise awareness of the consequences of different perspectivizations in the general public and in news producers alike.

==> tex/sec/interpret.tex <==
\section{Model Interpretation}

==> tex/sec/rsa.tex <==
\section{Representational Similarity Analysis}

==> tex/tab/explanations.tex <==
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lrrlrlrlrllrlr@{}}
\toprule
 & \multicolumn{6}{c}{\textbf{blame: murderer}} &  & \multicolumn{6}{c}{\textbf{focus: concept}} \\
 & \multicolumn{2}{c}{\textbf{ridge/bow}} & \multicolumn{2}{c}{\textbf{ridge/f1+}} & \multicolumn{2}{c}{\textbf{bertino}} &  & \multicolumn{2}{c}{\textbf{ridge/bow}} & \multicolumn{2}{c}{\textbf{ridge/f1+}} & \multicolumn{2}{c}{\textbf{bertino}} \\
 & \multicolumn{1}{l}{\textit{feature}} & \multicolumn{1}{l}{\textit{weight}} & \textit{feature} & \multicolumn{1}{l}{\textit{weight}} & \textit{token (context)} & \multicolumn{1}{l}{\textit{attr}} &  & \multicolumn{1}{l}{\textit{feature}} & \textit{weight} & \textit{feature} & \multicolumn{1}{l}{\textit{weight}} & \textit{token (context)} & \multicolumn{1}{l}{\textit{attr}} \\ \midrule
+1 & ex & \cellcolor[HTML]{57BB8A}0.38 & rol:Killing:Killer & \cellcolor[HTML]{57BB8A}0.21 & killer & \cellcolor[HTML]{7CCAA4}0.79 &  & che & \cellcolor[HTML]{57BB8A}0.20 & che & \cellcolor[HTML]{57BB8A}0.12 & femmini (-cidio) & \cellcolor[HTML]{A9DDC3}0.491 \\
+2 & uccide & \cellcolor[HTML]{57BB8A}0.33 & ex & \cellcolor[HTML]{57BB8A}0.15 & uccide & \cellcolor[HTML]{83CDA9}0.75 &  & pista & \cellcolor[HTML]{57BB8A}0.19 & sara & \cellcolor[HTML]{6EC49A}0.09 & figlio & \cellcolor[HTML]{C7E9D8}0.307 \\
+3 & moglie & \cellcolor[HTML]{57BB8A}0.31 & frm:Per\_rel & \cellcolor[HTML]{57BB8A}0.14 & assassino & \cellcolor[HTML]{89CFAD}0.71 &  & passionale & \cellcolor[HTML]{57BB8A}0.19 & pista & \cellcolor[HTML]{79C7A1}0.08 & non & \cellcolor[HTML]{DCF1E7}0.172 \\
+4 & uccise & \cellcolor[HTML]{57BB8A}0.24 & frm:Killing & \cellcolor[HTML]{57BB8A}0.13 & ex & \cellcolor[HTML]{99D6B8}0.62 &  & sara & \cellcolor[HTML]{57BB8A}0.19 & non & \cellcolor[HTML]{7DC9A4}0.08 & : & \cellcolor[HTML]{DDF2E8}0.166 \\
+5 & assassino & \cellcolor[HTML]{57BB8A}0.22 & cx:Pers\_rel++nvrb & \cellcolor[HTML]{57BB8A}0.13 & fidanzato & \cellcolor[HTML]{ABDDC5}0.51 &  & femminicidio & \cellcolor[HTML]{57BB8A}0.17 & femminicidio & \cellcolor[HTML]{7DC9A4}0.08 & suicidio & \cellcolor[HTML]{DFF2E9}0.154 \\
\rowcolor[HTML]{FFFFFF} 
{\color[HTML]{FFFFFF} } & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{FFFFFF} }} & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{FFFFFF} }} & {\color[HTML]{FFFFFF} } & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{FFFFFF} }} & {\color[HTML]{FFFFFF} } & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{FFFFFF} }} & {\color[HTML]{FFFFFF} } & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{FFFFFF} }} & {\color[HTML]{FFFFFF} } & {\color[HTML]{FFFFFF} } & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{FFFFFF} }} & {\color[HTML]{FFFFFF} } & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{FFFFFF} }} \\
-5 & sono & \cellcolor[HTML]{E67C73}-0.14 & rol:Event:Event & \cellcolor[HTML]{EBB0AB}-0.06 & una & \cellcolor[HTML]{FBEAE9}-0.14 &  & omicida & \cellcolor[HTML]{E67C73}-0.13 & nell' & \cellcolor[HTML]{EAA59F}-0.07 & uccisa & \cellcolor[HTML]{F7D9D7}-0.318 \\
-4 & della & \cellcolor[HTML]{E67C73}-0.15 & sono & \cellcolor[HTML]{EBADA7}-0.06 & . & \cellcolor[HTML]{FAE9E8}-0.14 &  & trovata & \cellcolor[HTML]{E67C73}-0.14 & della & \cellcolor[HTML]{EAA49E}-0.07 & morta & \cellcolor[HTML]{F7D9D6}-0.319 \\
-3 & - & \cellcolor[HTML]{E67C73}-0.16 & frm:Event & \cellcolor[HTML]{E99891}-0.08 & sono & \cellcolor[HTML]{FAE8E6}-0.15 &  & nell' & \cellcolor[HTML]{E67C73}-0.14 & due & \cellcolor[HTML]{EAA49E}-0.07 & killer & \cellcolor[HTML]{F6D0CD}-0.384 \\
-2 & accaduto & \cellcolor[HTML]{E67C73}-0.17 & della & \cellcolor[HTML]{E8928A}-0.08 & trovata & \cellcolor[HTML]{F9E3E1}-0.20 &  & ospedale & \cellcolor[HTML]{E67C73}-0.16 & cx:Buildings++nvrb & \cellcolor[HTML]{E99A93}-0.07 & auto & \cellcolor[HTML]{F5CDC9}-0.410 \\
-1 & . & \cellcolor[HTML]{E67C73}-0.35 & . & \cellcolor[HTML]{E67C73}-0.13 & morta & \cellcolor[HTML]{F9E1DF}-0.21 &  & due & \cellcolor[HTML]{E67C73}-0.16 & frm:Buildings & \cellcolor[HTML]{E7857D}-0.09 & uccide & \cellcolor[HTML]{F5CBC8}-0.421 \\ \bottomrule
\end{tabular}%
}
\caption{Comparison of most informative features / token attributions for an `easy' attribute (blame/murderer) and a `hard' attribute (focus/concept). [Abbreviations: rol=semantic role, frm=frame, cx=construction, nvrb=nonverbal, Pers\_rel=Personal\_relationship}
\end{table*}

==> tex/tab/results-overview-old.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% % \usepackage{graphicx}
% % \usepackage[table,xcdraw]{xcolor}
% % If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \begin{table*}[]
% \centering
% % \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}llrrrrrrrr@{}}
% \toprule
% \multicolumn{2}{c}{\textbf{model}} &
%   \multicolumn{3}{c}{\cellcolor[HTML]{CFE2F3}\textbf{direct}} &
%   \multicolumn{2}{c}{\cellcolor[HTML]{EAD1DC}\textbf{indirect}} &
%   \multicolumn{2}{c}{\cellcolor[HTML]{FFF2CC}\textbf{space}} \\
% \textit{model} &
%   \textit{features} &
%   \multicolumn{1}{l}{\cellcolor[HTML]{CFE2F3}\textit{RMSE}} &
%   \multicolumn{1}{l}{\cellcolor[HTML]{CFE2F3}\textit{R$^2$}} &
%   \multicolumn{1}{l}{\cellcolor[HTML]{CFE2F3}\textit{Cos}} &
%   \multicolumn{1}{l}{\cellcolor[HTML]{EAD1DC}\textit{Pair}} &
%   \multicolumn{1}{l}{\cellcolor[HTML]{EAD1DC}\textit{Rank}} &
%   \multicolumn{1}{l}{\cellcolor[HTML]{FFF2CC}\textit{NN}} &
%   \multicolumn{1}{l}{\cellcolor[HTML]{FFF2CC}\textit{RSA}} \\ \midrule
% {\color[HTML]{666666} baseline} &
%   {\color[HTML]{666666} mean} &
%   {\color[HTML]{666666} 0.66} &
%   {\color[HTML]{666666} -0.10} &
%   {\color[HTML]{666666} -0.06} &
%   {\color[HTML]{666666} *0.92} &
%   {\color[HTML]{666666} *0.50} &
%   {\color[HTML]{666666} *0.44} &
%   {\color[HTML]{666666} *-0.04} \\
% ridge &
%   surface-1 &
%   \cellcolor[HTML]{FFFFFF}0.64 &
%   \cellcolor[HTML]{F7FCFA}-0.02 &
%   \cellcolor[HTML]{F0F9F4}0.29 &
%   \cellcolor[HTML]{BFE5D3}0.79 &
%   \cellcolor[HTML]{E5F5ED}0.70 &
%   \cellcolor[HTML]{ECF8F2}0.51 &
%   \cellcolor[HTML]{FCFEFD}0.07 \\
% ridge &
%   surface-2 &
%   \cellcolor[HTML]{F8FCFA}0.63 &
%   \cellcolor[HTML]{FFFFFF}-0.03 &
%   \cellcolor[HTML]{FFFFFF}0.26 &
%   \cellcolor[HTML]{FFFFFF}0.73 &
%   \cellcolor[HTML]{FFFFFF}0.68 &
%   \cellcolor[HTML]{FFFFFF}0.49 &
%   \cellcolor[HTML]{FFFFFF}0.07 \\
% ridge &
%   theory-1a &
%   \cellcolor[HTML]{BBE3CF}0.60 &
%   \cellcolor[HTML]{C7E9D8}0.04 &
%   \cellcolor[HTML]{A3DABF}0.41 &
%   \cellcolor[HTML]{98D5B7}0.82 &
%   \cellcolor[HTML]{92D3B3}0.77 &
%   \cellcolor[HTML]{A6DBC1}0.55 &
%   \cellcolor[HTML]{ABDDC5}0.17 \\
% ridge &
%   theory-1b &
%   \cellcolor[HTML]{C6E7D7}0.60 &
%   \cellcolor[HTML]{BFE5D2}0.05 &
%   \cellcolor[HTML]{B2E0C9}0.38 &
%   \cellcolor[HTML]{9CD7BA}0.82 &
%   \cellcolor[HTML]{A2DABF}0.75 &
%   \cellcolor[HTML]{C6E8D8}0.53 &
%   \cellcolor[HTML]{B9E3CE}0.16 \\
% ridge &
%   theory-2a &
%   \cellcolor[HTML]{EBF6F1}0.62 &
%   \cellcolor[HTML]{E5F5ED}0.00 &
%   \cellcolor[HTML]{DBF1E6}0.32 &
%   \cellcolor[HTML]{C2E7D5}0.78 &
%   \cellcolor[HTML]{DCF1E7}0.70 &
%   \cellcolor[HTML]{D2EDE0}0.52 &
%   \cellcolor[HTML]{D1EDDF}0.13 \\
% ridge &
%   theory-2b &
%   \cellcolor[HTML]{E8F5EF}0.62 &
%   \cellcolor[HTML]{E0F3EA}0.01 &
%   \cellcolor[HTML]{CFECDE}0.34 &
%   \cellcolor[HTML]{B1E0C9}0.80 &
%   \cellcolor[HTML]{CDEBDC}0.72 &
%   \cellcolor[HTML]{BFE5D3}0.54 &
%   \cellcolor[HTML]{D9F0E4}0.12 \\
% ridge &
%   sentence-1 &
%   \cellcolor[HTML]{ACDDC5}0.59 &
%   \cellcolor[HTML]{BBE4D0}0.06 &
%   \cellcolor[HTML]{99D6B8}0.42 &
%   \cellcolor[HTML]{A5DBC1}0.81 &
%   \cellcolor[HTML]{7CCAA4}0.78 &
%   \cellcolor[HTML]{6DC49A}0.59 &
%   \cellcolor[HTML]{7BCAA3}0.23 \\
% ridge &
%   sentence-2 &
%   \cellcolor[HTML]{7FCBA6}0.56 &
%   \cellcolor[HTML]{6FC59B}0.16 &
%   \cellcolor[HTML]{70C59C}0.49 &
%   \cellcolor[HTML]{62C092}0.87 &
%   \cellcolor[HTML]{57BB8A}0.81 &
%   \cellcolor[HTML]{7FCBA6}0.58 &
%   \cellcolor[HTML]{68C296}0.26 \\
% ridge &
%   sentence-3 &
%   \cellcolor[HTML]{A4DABF}0.58 &
%   \cellcolor[HTML]{A1D9BE}0.09 &
%   \cellcolor[HTML]{8AD0AE}0.45 &
%   \cellcolor[HTML]{7BCAA3}0.84 &
%   \cellcolor[HTML]{75C89F}0.79 &
%   \cellcolor[HTML]{9BD7BA}0.56 &
%   \cellcolor[HTML]{93D4B4}0.20 \\
% BERT &
%   &
%   \cellcolor[HTML]{57BB8A}0.54 &
%   \cellcolor[HTML]{57BB8A}0.19 &
%   \cellcolor[HTML]{57BB8A}0.52 &
%   \cellcolor[HTML]{57BB8A}0.87 &
%   \cellcolor[HTML]{5DBE8E}0.81 &
%   \cellcolor[HTML]{57BB8A}0.61 &
%   \cellcolor[HTML]{57BB8A}0.28 \\ \bottomrule
% \end{tabular}%
% % 
% \caption{Development set results, 6-fold cross-validation. Lower is better for RMSE, higher is better for all others. Green coloring is calculated relative to best and worst scores within each column. (*) Indirect and Space scores are ill-defined for the baseline since all output vectors are the same. }\label{tab:results-overview}
% \end{table*}

==> tex/tab/results-r2-blame.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\centering
\resizebox{.5\textwidth}{!}{%
\begin{tabular}{@{}llrrrrrrr@{}}
\toprule
&&  \multicolumn{6}{c}{\textbf{R$^2$ for "the sentence puts the blame on..."}} \\ \midrule
\textbf{model} &
  \textbf{setup} &
  \multicolumn{1}{l}{\rotatebox[origin=c]{60}{\textit{murderer}}} &
  \multicolumn{1}{l}{\rotatebox[origin=c]{60}{\textit{victim}}} &
  \multicolumn{1}{l}{\rotatebox[origin=c]{60}{\textit{concept}}} &
  \multicolumn{1}{l}{\rotatebox[origin=c]{60}{\textit{object}}} &
  \multicolumn{1}{l}{\rotatebox[origin=c]{60}{\textit{no-one}}} &
  \multicolumn{1}{l}{{\color[HTML]{830ea0} \rotatebox[origin=c]{60}{mean}}} \\ \midrule
ridge &
  surface-1 &
  \cellcolor[HTML]{DFF2E9}0.09 &
  \cellcolor[HTML]{FFFFFF}-0.05 &
  \cellcolor[HTML]{FFFFFF}-0.11 &
  \cellcolor[HTML]{FFFFFF}-0.01 &
  \cellcolor[HTML]{AADDC4}0.09 &
  \cellcolor[HTML]{FCFEFD}{\color[HTML]{830ea0} 0.00} \\
ridge &
  surface-2 &
  \cellcolor[HTML]{FFFFFF}0.02 &
  \cellcolor[HTML]{FFFFFF}-0.11 &
  \cellcolor[HTML]{FFFFFF}-0.21 &
  \cellcolor[HTML]{FFFFFF}0.00 &
  \cellcolor[HTML]{FFFFFF}-0.01 &
  \cellcolor[HTML]{FFFFFF}{\color[HTML]{830ea0} -0.06} \\
ridge &
  theory-1a &
  \cellcolor[HTML]{C4E7D6}0.15 &
  \cellcolor[HTML]{FFFFFF}-0.06 &
  \cellcolor[HTML]{FFFFFF}-0.40 &
  \cellcolor[HTML]{57BB8A}0.26 &
  \cellcolor[HTML]{64C093}0.17 &
  \cellcolor[HTML]{D4EEE1}{\color[HTML]{830ea0} 0.02} \\
ridge &
  theory-1b &
  \cellcolor[HTML]{CCEADB}0.14 &
  \cellcolor[HTML]{FFFFFF}-0.02 &
  \cellcolor[HTML]{FFFFFF}-0.16 &
  \cellcolor[HTML]{83CDA9}0.19 &
  \cellcolor[HTML]{71C69C}0.15 &
  \cellcolor[HTML]{8ED1B0}{\color[HTML]{830ea0} 0.06} \\
ridge &
  theory-2a &
  \cellcolor[HTML]{D8F0E4}0.11 &
  \cellcolor[HTML]{FFFFFF}-0.07 &
  \cellcolor[HTML]{FFFFFF}-0.05 &
  \cellcolor[HTML]{A8DCC2}0.14 &
  \cellcolor[HTML]{FFFFFF}-0.08 &
  \cellcolor[HTML]{F0F9F5}{\color[HTML]{830ea0} 0.01} \\
ridge &
  theory-2b &
  \cellcolor[HTML]{D6EFE3}0.11 &
  \cellcolor[HTML]{FFFFFF}-0.05 &
  \cellcolor[HTML]{FFFFFF}-0.06 &
  \cellcolor[HTML]{D6EFE2}0.06 &
  \cellcolor[HTML]{C0E6D3}0.07 &
  \cellcolor[HTML]{CCEBDC}{\color[HTML]{830ea0} 0.03} \\
ridge &
  sentence-1 &
  \cellcolor[HTML]{7AC9A2}0.33 &
  \cellcolor[HTML]{FFFFFF}-0.01 &
  \cellcolor[HTML]{FFFFFF}-0.25 &
  \cellcolor[HTML]{FFFFFF}-0.19 &
  \cellcolor[HTML]{57BB8A}0.18 &
  \cellcolor[HTML]{EAF7F0}{\color[HTML]{830ea0} 0.01} \\
ridge &
  sentence-2 &
  \cellcolor[HTML]{8DD1AF}0.28 &
  \cellcolor[HTML]{FFFFFF}-0.06 &
  \cellcolor[HTML]{FFFFFF}-0.01 &
  \cellcolor[HTML]{FFFFFF}-0.06 &
  \cellcolor[HTML]{AFDFC8}0.09 &
  \cellcolor[HTML]{A9DCC3}{\color[HTML]{830ea0} 0.05} \\
ridge &
  sentence-3 &
  \cellcolor[HTML]{ACDEC5}0.21 &
  \cellcolor[HTML]{FFFFFF}-0.23 &
  \cellcolor[HTML]{57BB8A}0.06 &
  \cellcolor[HTML]{FFFFFF}-0.22 &
  \cellcolor[HTML]{A2DABE}0.10 &
  \cellcolor[HTML]{FFFFFF}{\color[HTML]{830ea0} -0.02} \\
BERT &
   &
  \cellcolor[HTML]{57BB8A}0.41 &
  \cellcolor[HTML]{FFFFFF}-0.12 &
  \cellcolor[HTML]{AADDC4}0.03 &
  \cellcolor[HTML]{F2FAF6}0.02 &
  \cellcolor[HTML]{91D3B3}0.12 &
  \cellcolor[HTML]{57BB8A}{\color[HTML]{830ea0} 0.09} \\ \bottomrule
\end{tabular}%
}
\caption{Per-dimension $R^2$ scores for \textit{blame} regression}\label{tab:results-r2-blame}
\centering
\end{table}

==> tex/tab/results-r2-focus.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\resizebox{.45\textwidth}{!}{%
\begin{tabular}{@{}llrrrrrr@{}}
\toprule
&&  \multicolumn{5}{c}{\textbf{R$^2$ for "the sentence focuses on..."}} \\ \midrule
\textbf{model} &
  \textbf{setup} &
  \multicolumn{1}{l}{\rotatebox[origin=c]{60}{\textit{murderer}}} &
  \multicolumn{1}{l}{\rotatebox[origin=c]{60}{\textit{victim}}} &
  \multicolumn{1}{l}{\rotatebox[origin=c]{60}{\textit{object}}} &
  \multicolumn{1}{l}{\rotatebox[origin=c]{60}{\textit{concept}}} &
  \multicolumn{1}{l}{{\color[HTML]{830ea0} \rotatebox[origin=c]{60}{mean}}} \\ \midrule
ridge &
  surface-1 &
  \cellcolor[HTML]{B2E0CA}0.19 &
  \cellcolor[HTML]{EEF8F3}0.04 &
  \cellcolor[HTML]{FFFFFF}-0.17 &
  \cellcolor[HTML]{FFFFFF}-0.13 &
  \cellcolor[HTML]{FFFFFF}{\color[HTML]{830ea0} -0.02} \\
ridge &
  surface-2 &
  \cellcolor[HTML]{BEE5D2}0.16 &
  \cellcolor[HTML]{F4FBF7}0.03 &
  \cellcolor[HTML]{FFFFFF}-0.17 &
  \cellcolor[HTML]{FFFFFF}-0.02 &
  \cellcolor[HTML]{FFFFFF}{\color[HTML]{830ea0} 0.00} \\
ridge &
  theory-1a &
  \cellcolor[HTML]{8DD1B0}0.28 &
  \cellcolor[HTML]{D3EDE0}0.11 &
  \cellcolor[HTML]{C3E7D5}0.17 &
  \cellcolor[HTML]{FFFFFF}-0.03 &
  \cellcolor[HTML]{C1E6D4}{\color[HTML]{830ea0} 0.13} \\
ridge &
  theory-1b &
  \cellcolor[HTML]{94D4B5}0.27 &
  \cellcolor[HTML]{C7E9D8}0.14 &
  \cellcolor[HTML]{EBF7F1}0.06 &
  \cellcolor[HTML]{FFFFFF}-0.03 &
  \cellcolor[HTML]{CDEBDC}{\color[HTML]{830ea0} 0.11} \\
ridge &
  theory-2a &
  \cellcolor[HTML]{D6EFE3}0.10 &
  \cellcolor[HTML]{D3EEE1}0.11 &
  \cellcolor[HTML]{FFFFFF}-0.06 &
  \cellcolor[HTML]{FFFFFF}-0.01 &
  \cellcolor[HTML]{EEF9F4}{\color[HTML]{830ea0} 0.04} \\
ridge &
  theory-2b &
  \cellcolor[HTML]{B2E0CA}0.19 &
  \cellcolor[HTML]{D3EEE1}0.11 &
  \cellcolor[HTML]{FFFFFF}-0.10 &
  \cellcolor[HTML]{FFFFFF}-0.09 &
  \cellcolor[HTML]{F3FAF7}{\color[HTML]{830ea0} 0.03} \\
ridge &
  sentence-1 &
  \cellcolor[HTML]{6CC499}0.36 &
  \cellcolor[HTML]{57BB8A}0.42 &
  \cellcolor[HTML]{FFFFFF}-0.13 &
  \cellcolor[HTML]{82CDA8}0.17 &
  \cellcolor[HTML]{9FD9BD}{\color[HTML]{830ea0} 0.21} \\
ridge &
  sentence-2 &
  \cellcolor[HTML]{84CDA9}0.31 &
  \cellcolor[HTML]{5ABC8C}0.42 &
  \cellcolor[HTML]{A8DCC3}0.24 &
  \cellcolor[HTML]{5DBE8E}0.21 &
  \cellcolor[HTML]{76C8A0}{\color[HTML]{830ea0} 0.29} \\
ridge &
  sentence-3 &
  \cellcolor[HTML]{61BF91}0.39 &
  \cellcolor[HTML]{70C59B}0.36 &
  \cellcolor[HTML]{E6F5EE}0.07 &
  \cellcolor[HTML]{57BB8A}0.22 &
  \cellcolor[HTML]{85CEAA}{\color[HTML]{830ea0} 0.26} \\
BERT &
   &
  \cellcolor[HTML]{57BB8A}0.41 &
  \cellcolor[HTML]{63C093}0.39 &
  \cellcolor[HTML]{57BB8A}0.47 &
  \cellcolor[HTML]{84CEAA}0.16 &
  \cellcolor[HTML]{57BB8A}{\color[HTML]{830ea0} 0.36} \\ \bottomrule
\end{tabular}%
}
\caption{Per-dimension $R^2$ scores for \textit{focus} regression}\label{tab:results-r2-focus}
\end{table}
